Lissy: Experimenting with on-chain order books

Financial regulators have long-standing concerns about fully decentralized exchanges that run 'on-chain' without any obvious regulatory hooks. The popularity of Uniswap, an automated market makers (AMM), made these concerns a reality. AMMs implement a lightweight dealer-based trading system, but they are unlike anything on Wall Street, require fees intrinsically, and are susceptible to front-running attacks. This leaves the following research questions we address in this paper: (1) are conventional (i.e., order books), secure (i.e., resistant to front-running and price manipulation) and fully decentralized exchanges feasible on a public blockchain like Ethereum, (2) what is the performance profile, and (3) how much do Layer 2 techniques (e.g., Arbitrum) increase performance? To answer these questions, we implement, benchmark, and experiment with an Ethereum-based call market exchange called Lissy. We confirm the functionality is too heavy for Ethereum today (you cannot expect to exceed a few hundred trade executions per block) but show it scales dramatically (99.88% gas cost reduction) on Arbitrum.

==> tables/AMMvsLOB.tex <==
% !TEX root = ../main.tex

% = = = = = = = = = = = = = = = = = = = = =Call market operations Table = = = = = = = = = = = =  = = = = = =  %
\begin{table}[t]
%\setlength{\tabcolsep}{0.7\tabcolsep}% Shrink \tabcolsep

\centering
\footnotesize
\begin{tabular}{|>{\centering}m{2.2cm} |>{\centering\arraybackslash}m{9cm}|}%{|c|c|}

\hline
\multicolumn{1}{|c|}{\textbf{Operation}} & \multicolumn{1}{c|}{\textbf{Description}}                            			\\ \hline

% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %
	depositToken()                           & Deposits ERC20 tokens in \cm smart contract \\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %
	depositEther()                           	& Deposits ETH in \cm smart contract                        			 \\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %
	openMarket()                             & Opens the market                                                    					 \\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %
	closeMarket()                            & Closes the market and processes the orders       \\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %
	submitBid()                              & Inserts the upcoming bids inside the priority queue   \\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %
	submitAsk()                              & Inserts the upcoming asks inside the priority queue  \\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %
	claimTokens()                           & Transfers tokens to the traders                       			\\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %
	claimEther()                             & Transfers ETH to the traders                       			\\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %
\end{tabular}
\caption{Primary operations of \cm smart contract.
\label{tab:cm_functions}}
\end{table}

% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %

==> tables/dequeue.tex <==
% !TEX root = ../main.tex

% = = = = = = = = = = = =Gas costs and refunds for Dequeueing 50 integers from each PQ  = = = = = = = = = = = = =  %

\begin{table}[t]
\setlength{\tabcolsep}{0.2\tabcolsep}% Shrink \tabcolsep
\centering
\begin{tabular}{|c|c|c|l|}

\multicolumn{1}{c}{} & \headrow{\footnotesize Gas Costs (\texttt{gasUsed})} & \headrow{\footnotesize Potential Refund} & \headrow{\footnotesize Full Refund?} \\ \hline

% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
Heap with Dynamic Array       	& 2,518,131          & 750,000     &\full                  \\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
Heap with Static Array          	& 1,385,307                             & 750,000      &\full                \\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
Heap with Mapping 			& 2,781,684                            & 1,500,000    &\full                 \\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
Linked List                     		& 557,085               	           & 1,200,000      &\full                \\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
Linked List with Mapping      	& 731,514              	     	  &  3,765,000      &\full                 \\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %

\end{tabular}
\caption{The gas metrics associated with dequeuing 50 integers from five priority queue variants. For the refund, (\full) indicates the  refund was capped at the maximum amount and (\prt) means a greater refund would be possible.
\label{tab:PQUnitTests}}
\end{table}
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %


% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %
%  = = = = = = Table 2 (dequeue) Conversions = = = = = = %
%
%As of July 2020,  $1 gas = 56\times10^{-9} ether$\footnote{https://ethstats.net/} and 1 ether = \$238.33\footnote{https://coinmarketcap.com/}.
%
%$Transaction cost (eth) = GasUsed (unit) \times Gas Price (eth)$ 
%
%%  = = = = = = Transaction Costs in eth = = = = = = %
%
%Heap with Dynamic Array:    		$2,518,131 \times 56\times10^{-9} = 141,015,336\times 10^{-9}$
%Heap with Dynamic Array:     		$1,385,307 \times 56\times10^{-9} = 77,577,192\times 10^{-9}$
%Heap with Mapping:              		$2,781,684 \times 56\times10^{-9} = 155,774,304\times 10^{-9}$
%Linked List:						$557,085 \times 56\times10^{-9} = 	31,196,760\times 10^{-9}$
%Linked List with Mapping:			$731,514 \times 56\times10^{-9} = 	40,964,784\times 10^{-9}$
%
%%  = = = = = = Transaction Costs in USD = = = = = = %
%
%Heap with Dynamic Array:    		$141,015,336\times 10^{-9} \times 238.33 = \$33.60$
%Heap with Dynamic Array:     		$77,577,192\times 10^{-9} \times 238.33 = \$18.48$
%Heap with Mapping:              		$155,774,304\times 10^{-9} \times 238.33 = \$37.12$
%Linked List:						$31,196,760\times 10^{-9} \times 238.33 = \$7.43$
%Linked List with Mapping:			$40,964,784\times 10^{-9} \times 238.33 = \$9.76$
%
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %


==> tables/eval.tex <==
% !TEX root = ../main.tex



\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\multicolumn{1}{c}{} &
%Security
\headrow{Non-Custodial} &
\headrow{\shortstack{No Trusted \\Third Party}} & 
\headrow{Fully Autonomous} & 


%Deployability
\headrow{\shortstack{Resilient to\\ Server Downtime}} & 
\headrow{\shortstack{Resilient to Ethereum \\ Network Congestion}} & 
\headrow{High Trade Performance} &

%Market Characteristics
\headrow{Certain Fulfillment} &
\headrow{Low Price Slippage} &
\headrow{No Impermanent Loss} &
\headrow{T+0 Settlement} 






\\
\hline

%
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %

\multicolumn{1}{|c}{\textbf{Exchange Platform}} 			& \multicolumn{3}{|c}{\textbf{\shortstack{Security\\ Properties}}} &		\multicolumn{3}{|c}{\textbf{\shortstack{Deployability \\Properties}}} & 		\multicolumn{4}{|c|}{\textbf{\shortstack{Market \\Characteristics}}}  \\ \cmidrule[0.7mm]{1-11}
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
\shortstack{Centralized Continuous\\ Market \textit{(CEX)}}				&\empt			&\empt		&\empt			&	\empt	&\full		&\full		&\empt		&\full		&\full 		&\empt		\\ \hline	

% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
\shortstack{Partially Off-chain \\Continuous Market \textit{(DEX)}}			&\prt 	&\prt		&\prt			&\empt		&\prt 		&\full		&\empt 		&\full 		&\full		&\full		\\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
\shortstack{Partially Off-chain \\Continuous Market w/ Roll-up}    						&\full			&\full			&\empt 		 		&\empt 		&\prt		&\prt		&\empt 	&\full			&\full			&\full	 		\\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
On-chain Continuous Market			&\full			&\full			&\full			&\full			&\empt  		&\empt 		&\empt 		&\full			&\full			&\full			\\ \hline

% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
\shortstack{On-chain Automated \\Market Maker}		&\full			&\full			&\full				&\full			&\empt 	&\empt 	&\full			&\empt 		&\empt 		&\full			\\  \hline

% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
On-chain Call Market   					&\full			&\full			&\full				&\full			&\empt 	&\empt 		&\empt 	&\full			&\full			&\full			\\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %

\shortstack{On-chain Call Market\\ w/ Roll-up}		 	&\full			&\full			&\empt 			&\empt 	&\prt		&\prt		&\empt 	&\full			&\full			&\full			\\ \hline


\hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %


\end{tabular}
\caption{\footnotesize{Comparative evaluation of different types of exchange platforms: {\full} indicates the properties (columns) are fulfilled by the corresponding mechanism (rows) within reason, {\empt} means the property is not fulfilled, \textblue{and {\prt} means the property is partially fulfilled.}}
\label{tab:eval}}
\end{table*}

	

==> tables/frontrunning.tex <==
% !TEX root = ../main.tex


%\begin{adjustbox}{center} %horizontal display
\begin{landscape} %vertical display
\begin{table}[t]
\setlength{\tabcolsep}{3\tabcolsep}
\centering

\footnotesize

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\headrowfront{\scriptsize{Centralized Continuous Market (Coinbase)}} &
\headrowfront{\scriptsize{Partially Off-chain Continuous Market (EtherDelta)} } & 
\headrowfront{\scriptsize{Partially Off-chain Continuous Market w/ Roll-up (Loopring)} } & 
\headrowfront{\scriptsize{On-chain Continuous Market (OasisDex)} } &
\headrowfront{\scriptsize{On-chain Dark Continuous Market (TEX)} }&
\headrowfront{\scriptsize{On-chain Automated Market Maker (Uniswap)} } & 
\headrowfront{\scriptsize{On-chain Call Market w/ Price Improvement}} &
\headrowfront{\scriptsize{On-chain Call Market (\cm)}}  & 
\headrowfront{\scriptsize{On-chain Call Market w/ Roll-up (\cm variant)}}  &
\headrowfront{\scriptsize{On-chain Dark Call Market (Galal \etal)}} 
\\

%\hhline{-----------}
\hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %								 											
%\parbox[t]{1mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{Attack Example}}} 	&&&&&&&&&&&														\\ \hline		
	     
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %								 											
	     
%	     
%	     & \multicolumn{2}{c?{1mm}}{Classification}             																											&\multicolumn{1}{c|}{LOB}		&\multicolumn{1}{c|}{LOB}		&\multicolumn{1}{c|}{LOB}		&\multicolumn{1}{c|}{LOB}		&\multicolumn{1}{c|}{LOB}		&\multicolumn{1}{c|}{AMM}		&\multicolumn{1}{c|}{CM}		&\multicolumn{1}{c|}{CM}	&\multicolumn{1}{c|}{CM}								  										&\multicolumn{1}{c|}{CM}	 \\ \hhline{~------------}                 

% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %								 											

\multicolumn{3}{|c?{1mm}}{\makecell{Who is Mallory? \\ \underline{A}uthority,  \underline{T}rader, \underline{M}iner, \underline{S}equencer	}}   	&A&A,T,M&A,T,M,S&T,M&T,M&T,M&T,M&T,M&T,M,S	&T,M	 \\ \cmidrule[1mm]{1-13}

% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %								 											

\multirow{17}{*}{\rotatebox[origin=c]{90}{\textbf{Attack Example}}}		&\multicolumn{1}{c|}{\makecell{Mallory (\textit{maker}) squeezes in a\\ transaction before Alice's  (\textit{taker})  order}}  						&\multicolumn{1}{c?{1mm}}{Ins.}		&\empt	&\empt &\empt &\empt &\full &\empt &\full &\full  &\full &\full		\\ \hhline{~------------}					 					
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %								 											
								 											
&\multicolumn{1}{c|}{\makecell{Mallory (\textit{taker}) squeezes in a \\transaction before Bob's (\textit{taker 2})}   }	  								&\multicolumn{1}{c?{1mm}}{  Disp.}				&\empt &\empt &\empt &\empt &\full &\empt &\full &\full &\full	&\full		\\ \hhline{~------------}	
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %

&\multicolumn{1}{c|}{\makecell{Mallory (\textit{maker 1}) suppresses a better \\ incoming order from Alice (\textit{maker 2}) \\ until Mallory's order is executed}}																&\multicolumn{1}{c?{1mm}}{Supp.} 				&\empt &\empt &\empt &\full &\full &\full &\prt &\prt &\prt &\prt	\\ 	\hhline{~------------}				 											
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %

&\multicolumn{1}{c|}{\makecell{A hybrid attack based on the above \\ (\eg sandwich attacks, scalping)}}																		&\multicolumn{1}{c?{1mm}}{I/S/D}																		&\empt &\empt &\empt &\empt &\full &\empt &\empt &\full &\full	&\full												\\ 	\hhline{~------------}
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %

&\multicolumn{1}{c|}{\makecell{Mallory suspends the market \\for a period of time}}																										&\multicolumn{1}{c?{1mm}}{Supp.}    				&\empt  &\empt  &\empt  &\prt  &\prt  &\prt  &\prt  & \prt &\prt &\prt 	\\ 	\hhline{~------------}
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %

&\multicolumn{1}{c|}{\makecell{Spoofing: Mallory (\textit{maker}) puts an \\ order as bait, sees Alice (\textit{taker}) \\ tries to execute it, and cancels it first}}													&\multicolumn{1}{c?{1mm}}{S\&D} 				&\empt &\empt &\empt &\empt &\full &\empt &\full &\full &\full &\full \\ 	\hhline{~------------}
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %

&\multicolumn{1}{c|}{\makecell{Cancellation Griefing: Alice (\textit{maker}) \\ cancels an order and Mallory \\ (\textit{taker}) fulfills it first}}													&\multicolumn{1}{c?{1mm}}{Disp.} 							&\empt &\empt &\empt &\empt &\full &\empt &\full & \full &\full	&\full \\ 	\hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = == = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %



\end{tabular}

%} %end resizebox




%\end{adjustbox}


\caption{An evaluation of front-running attacks (rows) for different types of order books (columns). Front-running attacks are in three categories: \underline{Ins}ertion, \underline{disp}lacement, and \underline{supp}ression. A full dot (\full) means the front-running attack is mitigated or not applicable to the order book type, a partial mitigation (\prt) is awarded when the front-running attack is possible but expensive, and we give no award (\empt) if the attack is feasible. 
\label{tab:front}}
\end{table}

\end{landscape} 



==> tables/pq.tex <==
% !TEX root = ../main.tex

% = = = = = = = = = = = =Operations for a generic Priority Queue Table = = =  = = = = = = = = = = = %
\begin{table}[t]
%\setlength{\tabcolsep}{1pt}% Shrink \tabcolsep
\centering
\scriptsize
\begin{tabular}{|c|c|}
\hline

\textbf{Operation}   & \textbf{Description}    \\ \hline

% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
	\textbf{Enqueue()}       	& Inserts an element into the priority queue                        \\ \hline
	\textbf{Dequeue()}		& Removes and returns the highest priority element 		\\ \hline
	\textbf{isEmpty()}			& Checks if the priority queue is empty 					\\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %

\end{tabular}
\caption{\footnotesize{Operations for a generic priority queue}.
\label{tab:PQ_API}}
\end{table}
% = = = = = = = = = = = = = = = = = = = = =  = = = = = = = = = = =  = = = = = = = = = == = = =  = =%

==> tables/tradeexecutions.tex <==
% !TEX root = ../main.tex

% = = = = = = = = = = = =Comparison Trade Executions = = =  = = = = = = = = = = = %
\begin{table}[t]
%\setlength{\tabcolsep}{1pt}% Shrink \tabcolsep
\centering
\scriptsize
%\begin{tabular}{|c|c|c|c|c|}
\begin{tabular}{|>{\centering}m{4.5cm} |>{\centering}m{1cm} |>{\centering}m{1cm} |>{\centering}m{1cm} |>{\centering\arraybackslash}m{1cm}|}

\multicolumn{1}{c}{\scriptsize{Trade Execution System}}  & \headrowcleaning{\scriptsize {High Performance}} & \headrowcleaning{\scriptsize {High Security}} & \headrowcleaning{\scriptsize {Easy to Regulate}} & \headrowcleaning{\scriptsize {Easy to Realize}}\\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = %
	\textbf{Centralized Exchange (CEX)}       		 & \footnotesize\Smiley     	&\footnotesize\Sadey 		&\footnotesize\Smiley 		& \footnotesize\Smiley                 \\ \hline
	\textbf{Decentralized Exchange (DEX)}		 &\footnotesize\Smiley 		&\footnotesize\Sadey 		&\footnotesize\Smiley 		&\footnotesize\Smiley		\\ \hline
	\textbf{Fully On-chain Exchange}			 &\footnotesize\Sadey 		&\footnotesize\Smiley 		&\footnotesize\Sadey 		&\footnotesize\Sadey					\\ \hline
% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =  %
\end{tabular}
\caption{\footnotesize{}.
\label{tab:exchanges}}
\end{table}
% = = = = = = = = = = = = = = = = = = = = =  = = = = = = = = = = =  = = = = = = = = = == = = =  = =%
